FAME: Flexible, Scalable Analogy Mappings Engine

Analogy is one of the core capacities of human cognition; when faced with new situations, we often transfer prior experience from other domains. Most work on computational analogy relies heavily on complex, manually crafted input. In this work, we relax the input requirements, requiring only names of entities to be mapped. We automatically extract commonsense representations and use them to identify a mapping between the entities. Unlike previous works, our framework can handle partial analogies and suggest new entities to be added. Moreover, our method's output is easily interpretable, allowing for users to understand why a specific mapping was chosen. Experiments show that our model correctly maps 81.2% of classical 2x2 analogy problems (guess level=50%). On larger problems, it achieves 77.8% accuracy (mean guess level=13.1%). In another experiment, we show our algorithm outperforms human performance, and the automatic suggestions of new entities resemble those suggested by humans. We hope this work will advance computational analogy by paving the way to more flexible, realistic input requirements, with broader applicability.

==> 2problem/constraints/constraints.tex <==
\begin{itemize}
    \item Entities from the base (or target) should be mapped to at most one entity from the target (or base). 
    % Notice that there is no guarantee that each entity will be mapped. 
  \item Entities should be nouns and consist of at most two tokens.
%   \item one-to-one constraint: requires that each entity from the base would be mapped to at most one entity from the target and vice-verse. Notice that there is no guarantee that each entity will maps. 
%   \item Entities should be nouns and consist of at most two tokens.
\end{itemize}

==> 2problem/notation/kernel.tex <==
Given the structure of one or more single-mappings, if this structure is consistent, it will be marked as a kernel. A consistent structure means that the single-mappings that make it up are consistent and do not contradict each other. Example for inconsistent structure: given the following two single-mapping: $\{b_1$:$b_2 \sim t_1$:$t_2$, $b_1$:$b_3 \sim t_2$:$t_3\}$, from the first we conclude that $b_1$ $\rightarrow$ $t_1$ and $b_2$ $\rightarrow$ $t_2$,  but from the second we conclude that $b_1$ $\rightarrow$ $t_2$ and $b_3$ $\rightarrow$ $t_3$, and it is clear that the mappings here are inconsistent. Each kernel receives a structure evaluation score, which is detailed later. 

==> 2problem/notation/relations.tex <==
Given two entities $ e_1, e_2, $ the relations between them will be marked as $R(e_1,e_2)$. For example, if the set of relations between \textit{earth} and \textit{sun} are \{revolve around, attracted to\}, it will be marked as $R(earth, sun)$. Notice that the order is important, due to the asymmetric of the function. For example, Newton discovered gravity, but gravity did not discover Newton.

==> 2problem/notation/single-mapping.tex <==
Given two entities from the base $b_1$, $b_2$ and two entities from the target $t_1$, $t_2$, the function that maps $b_1$ $\rightarrow$ $t_1$ and $b_2$ $ \rightarrow$ $t_2$ will be symmetrically marked as $b_1$:$b_2 \sim t_1$:$t_2$. For example, the meaning of $sun$:$earth$ $\sim$ $nucleus$:$electrons$ is that we map sun $\rightarrow$ nucleus and earth $\rightarrow$ electrons.\remove{ According to that marking, $b_1$:$b_2 \sim t_1$:$t_2$ is equivalent to $b_2$:$b_1 \sim t_2$:$t_1$.} While the marking we present here describes a partial mapping from  \base to \targ, any such single-mapping also holds a score presented in the problem definition as relational similarity $sim^*$, which is detailed later.
